Memento: Long-Horizon Reasoning in Video Generation by Writing States into Pixels

Video generation models can solve reasoning problems in pixels, but their success collapses as the reasoning horizon - the number of dependent steps a problem takes - grows. A single generation denoises all frames jointly, so no intermediate result is fixed before the steps that depend on it are computed. We propose Memento. Its visible cache renders the hidden state of the process - a running sum, the pose of an object, the velocity of a ball - into the frame. Its chain of passes generates the video in short passes, each conditioned only on the last frame of the previous pass and the unchanged instruction, so every pass starts from a frame that shows everything computed so far and takes only the next step. Memento requires no architectural change, only image-to-video fine-tuning on videos rendered with a task-specific cache; at inference the model receives just the first frame and the instruction, and writes and reads the cache itself. On six procedurally generated tasks in arithmetic, spatial and physical reasoning, with the horizon controlled, Memento raises average success at horizon 4 from 0.16 for standard single-pass generation to 0.66 on Wan2.2-TI2V-5B, and retains 0.54 at horizon 8, where the single pass falls to 0.07; the gains at horizon 4 carry over to LongCat-Video. Gains are largest where a plain frame hides the whole state and smallest on the physical tasks, where it hides only the velocity. With the training instances and the number of frames held fixed, the cache without the chain and the chain without the cache both fall short of Memento on every task and on both base models tested.

==> figures/teaser.tex <==
\makeatletter
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
  \def\@captype{figure}
  \includegraphics[width=1\linewidth]{figures/teaser_fig.pdf}
  \vspace{-1.2em}
\caption{\textbf{Single pass versus Memento} on a waypoint maze ($N{=}4$): the ball must visit waypoints 1--4 in order. \emph{Top:} a single pass generates all 193 frames jointly; the ball reaches waypoints 1--3, then loops between 2 and 3 and never reaches 4. \emph{Bottom:} Memento generates as many frames as a chain of four passes, one per waypoint. Each later pass is conditioned only on the last frame of the previous one and the unchanged instruction. The visible cache (teal trail) is generated by the model and marks the visited cells, so each pass reads from its first frame where the ball has been; the ball reaches all four waypoints in order. The faint red path is overlaid for display only.}
  \label{fig:teaser}
\end{center}
}]
\makeatother

